Towards Faster Non-Asymptotic Convergence for Diffusion-Based Generative Models

Diffusion models, which convert noise into new data instances by learning to reverse a Markov diffusion process, have become a cornerstone in contemporary generative modeling. While their practical power has now been widely recognized, the theoretical underpinnings remain far from mature. In this work, we develop a suite of non-asymptotic theory towards understanding the data generation process of diffusion models in discrete time, assuming access to $\ell_2$-accurate estimates of the (Stein) score functions. For a popular deterministic sampler (based on the probability flow ODE), we establish a convergence rate proportional to $1/T$ (with $T$ the total number of steps), improving upon past results; for another mainstream stochastic sampler (i.e., a type of the denoising diffusion probabilistic model), we derive a convergence rate proportional to $1/\sqrt{T}$, matching the state-of-the-art theory. Imposing only minimal assumptions on the target data distribution (e.g., no smoothness assumption is imposed), our results characterize how $\ell_2$ score estimation errors affect the quality of the data generation processes. In contrast to prior works, our theory is developed based on an elementary yet versatile non-asymptotic approach without resorting to toolboxes for SDEs and ODEs. Further, we design two accelerated variants, improving the convergence to $1/T^2$ for the ODE-based sampler and $1/T$ for the DDPM-type sampler, which might be of independent theoretical and empirical interest.

==> other_preliminary.tex <==

\section{Other preliminaries}

, while the reverse process is learned by learning proper parametrization of the transition kernels. 




In order to generate new data samples, DDPMs start by generating a pure noise vector followed by running a pre-trained Markov chain in the reverse
time direction, which gradually turns the noise vector into a targeted structured distribution. 
The reverse process is also a Markov chain that we aim to learn using the data samples. 
Specifically, learning the reverse process corresponds to model the distribution of $X_{T}$ and also the transition kernel $P(X_{t-1}\mymid X_t)$ for $1 \leq t \leq T$ as   
\begin{align*}
	P(X_0, X_1, \ldots, X_T) &= P(X_0\mymid X_1, \ldots, X_T)P(X_1\mymid X_2, \ldots, X_T)\ldots P(X_{T-1}\mymid X_T) P(X_T) \\
	&= P(X_0\mymid X_1)P(X_1\mymid X_2)\cdots P(X_{T-1}\mymid X_T)P(X_T),
\end{align*}
since $P(X_{t-1} \mymid X_t, \ldots, X_T) = P(X_{t-1} \mymid X_t, W_{t+1}, \ldots, W_T) = P(X_{t-1} \mymid X_t)$.
As shall be discussed in more details, the idea is to approximate the reverse process by generating $Y_{T}$ from $\mathcal{N}(0,I_d)$ and 
approximate the reverse transition kernel $P(X_{t-1}\mymid X_t = x_t)$ by a Gaussian distribution
\begin{align}
\label{eqn:learned-rp}
	Y_{t-1} \mid Y_t = x_t \sim \mathcal{N}(\mu_{\theta}(x_t, t), \Sigma_{\theta}(x_t, t))
\end{align}
to match the actual time reversal of the forward Markov chain. 
Here and throughout this paper, to make our exposition clear, random variables that follow the distributions of the estimated Markov chain are denoted using $Y_{t}$, for $1\leq t\leq T.$
Our goal is to find the parametrization $\theta$ in expression~\eqref{eqn:learned-rp} such that $P(X_1,\ldots,X_T)$ is as close to $P(Y_1,\ldots,Y_T)$ as possible. Our theory aims to provide a mathematical characterization about how well $Y_{0}$ which is sampled recursively from \eqref{eqn:learned-rp} approximates the target distribution of $X_{0}$.

\paragraph{Training DDPM.} 
% \begin{align}
% 	X_t \mid X_0 = x_0 \sim \mathcal{N}\big(\sqrt{\overalpha_t}x_0, (1 - \overalpha_t)I_d\big)
% \end{align}

Let us write the density functions for $P(X_0, X_1, \ldots, X_T)$ as $q(x_0, x_1, \ldots, x_T)$ and that of $P_\theta(Y_0, Y_1, \ldots, Y_T)$ as $p_\theta(x_0, x_1, \ldots, x_T)$.
Our goal is to find the parametrization $\theta$ such that the KL divergence between the joint distributions of the data samples and the learned reverse process is minimized. 
It is equivalent to minimize 
\begin{align*}
	\kl(P(X_0, X_1, \ldots, X_T) \mid\mid P_\theta(Y_0, Y_1, \ldots, Y_T))
	&=
	\int \log \frac{q(x_0, x_1, \ldots, x_T)}{p_\theta(x_0, x_1, \ldots, x_T)} \mathsf{d} q(x_0, x_1, \ldots, x_T) \\
	%
	&= - \Exs_{q(x_0, x_1, \ldots, x_T)} \Big[\log p_\theta(X_0, X_1, \ldots, X_T)\Big] + \text{const} \\
	%
	&= -\Exs_{q(x_0, x_1, \ldots, x_T)}  \Big[\log p_\theta(X_T) + \sum_{t=1}^T \log \frac{p_\theta(X_{t-1} \mid X_t)}{q(X_{t-1} \mid X_t)} \Big] + \text{const} \\
	%
	&=  \sum_{t=1}^T  \Exs_{q(x_0, x_1, \ldots, x_T)}  \Big[ \log \frac{q(X_{t} \mid X_{t-1})}{p_\theta(X_{t-1} \mid X_t)} \Big] + \text{const}.
	%
\end{align*}
The first term on right hand side is often referred to as the variational bound for $\Exs[-\log p_\theta(X_0)]$. To further control the right hand side, the first term on the right can be rewritten as (\cite{ho2020denoising})  
\begin{align*}
	&\Exs_q \Big[\kl(q(X_T \mid X_0) ~||~ p(X_T)) + \sum_{T> t > 1}\kl(q(X_{t-1} \mid X_{t}, X_0) ~||~ p_{\theta}(X_{t-1}\mid X_t)) - \log p_{\theta}(X_0\mid X_1)\Big].
%
	% &= \Exs_q \Big[\int \log \frac{q(x_T \mid X_0)}{p(x_T)} q(x_T \mid X_0)\Big]
	% +
	%  \sum_{t > 1} \Exs_q \Big[\int \log \frac{q(x_{t-1} \mid X_T, X_0)}{p_\theta(x_{t-1} \mid X_T)} q(x_{t-1} \mid X_T, X_0)\Big] - \Exs_q \Big[\log p_{\theta}(X_0\mid X_1)\Big]\\ 
\end{align*}
It thus sufficient to select $\theta$ in order to minimize $\kl(q(X_{t-1} \mid X_{t}, X_0) ~||~ p_{\theta}(X_{t-1}\mid X_t))$ for each $1 < t < T.$
Towards this, in view of the properties of Gaussian distributions, conditional on $X_{0}$ and $X_{t}$, the distribution of $X_{t-1}$ obeys 
\begin{align}
	q(X_{t-1} \mid X_{t}, X_0) \sim \mathcal{N}(\widetilde{\mu}_t, \widetilde{\beta}_t I_d)
\end{align}
with 
\begin{align*}
	\widetilde{\mu}_t = \frac{\sqrt{\overalpha_{t-1}} (1-\alpha_t)}{1-\overalpha_{t}}X_0 + \frac{\sqrt{\alpha_{t}} (1-\overalpha_{t-1})}{1-\overalpha_{t}}X_t
	\qquad
	\text{and}
	\qquad
	\widetilde{\beta}_t = \frac{1 - \overalpha_{t-1}}{1 - \overalpha_{t}}(1-\alpha_t).
\end{align*}
Taking $p_{\theta}(X_{t-1}\mid X_t) \sim \mathcal{N}(\mu_{\theta}(x_t, t), \sigma_t^2I_d)$ with $\sigma_t^2 = \widetilde{\beta}_t$, in order to minimize $\kl(q(X_{t-1} \mid X_{t}, X_0) ~||~ p_{\theta}(X_{t-1}\mid X_t))$,
it then boils down to use $\mu_{\theta}(x_t, t)$ to approximate $\widetilde{\mu}_t$.
Recognizing the relation~\eqref{eqn:Xt-X0} where
\begin{align*}
	X_t = \sqrt{\overalpha_t} X_{0} + \sqrt{1-\overalpha_t} ~\overW_{t},
\end{align*}
it is then sufficient to use $X_{t}$ to predict $\overW_{t}$.


Based on the above intuition, for training DDPM, the common procedure seeks for a parameterization $s_{\theta}$ such that 
\begin{align}
\label{eqn:theta-training}
	\min_{\theta} \sum_t \mathbb{E}_{W\sim\mathcal{N}(0, I), X_0 \sim p_{X_0}} \Big[\|W - s_{\theta}(\sqrt{\overline{\alpha}_t} X_0 + \sqrt{1-\overline{\alpha}_t}W, t)\|^2\Big].
\end{align}
Given an estimator $\widehat{\theta}$ to the above optimization problem, for each $1\leq t \leq T$, the sampling proceeds 
\begin{align}
	Y_{t-1} = \frac{1}{\sqrt{\alpha_t}}\Big(Y_t - \frac{1-\alpha_t}{\sqrt{1-\overline{\alpha}_t}}s_{\widehat{\theta}}(Y_t, t)\Big) + \sigma_{t} W_t, 
	\qquad
	Y_T \sim \mathcal{N}(0, I_d),
\end{align}
with
\begin{align*}
\sigma_{t}^{2} = \frac{1 - \overalpha_{t-1}}{1 - \overalpha_{t}}(1-\alpha_t).
\end{align*}
The above procedure yields the same form as of the training for Score-Based Generative Models (SGMs), where the goal therein is to estimate the distribution and perform efficient sampling via the score functions $\nabla_{x_t}\log q(x_t).$ See \cite{yang2022diffusion} for more details. 
% This is closely related to Langevin dynamics:
% \begin{align*}
% X_t = X_{t-1} + \frac{\delta}{2}\nabla\log p_0(X_{t-1}) + \sqrt{\delta}W_t.
% \end{aog T)$.



